Prioritized Garbage Collection: Explicit GC Support for Software Caches

Programmers routinely trade space for time to increase performance, often in the form of caching or memoization. In managed languages like Java or JavaScript, however, this space-time tradeoff is complex. Using more space translates into higher garbage collection costs, especially at the limit of available memory. Existing runtime systems provide limited support for space-sensitive algorithms, forcing programmers into difficult and often brittle choices about provisioning. This paper presents prioritized garbage collection, a cooperative programming language and runtime solution to this problem. Prioritized GC provides an interface similar to soft references, called priority references, which identify objects that the collector can reclaim eagerly if necessary. The key difference is an API for defining the policy that governs when priority references are cleared and in what order. Application code specifies a priority value for each reference and a target memory bound. The collector reclaims references, lowest priority first, until the total memory footprint of the cache fits within the bound. We use this API to implement a space-aware least-recently-used (LRU) cache, called a Sache, that is a drop-in replacement for existing caches, such as Google's Guava library. The garbage collector automatically grows and shrinks the Sache in response to available memory and workload with minimal provisioning information from the programmer. Using a Sache, it is almost impossible for an application to experience a memory leak, memory pressure, or an out-of-memory crash caused by software caching.

==> Makefile <==
MAIN 			:= paper

PDFLATEX  := pdflatex -halt-on-error -interaction nonstopmode
BIBTEX		:= bibtex

TEX      := $(wildcard *.tex)
BIB      := $(wildcard *.bib)
RSCRIPTS := $(wildcard r/*.r)
PLOTS    := $(patsubst r/%.r,plots/%.pdf,$(RSCRIPTS))
FIGS     := $(wildcard figures/*.pdf)
OUTPUT   := $(addsuffix .pdf,$(MAIN))
AUX      := $(addsuffix .aux,$(MAIN))

FIND_BIB_CMD := grep -l \\\\bibliography{ $(TEX)
TEX_WITH_BIB := $(shell $(FIND_BIB_CMD) )
BBL 	       := $(TEX_WITH_BIB:.tex=.bbl)

SIDE_EFFECTS := $(OUTPUT) $(AUX) $(BBL) \
							 	$(addsuffix .out,$(MAIN)) \
							 	$(addsuffix .blg,$(MAIN)) \
							 	$(addsuffix .log,$(MAIN))

all: $(AUX) $(BIB) $(BBL) $(OUTPUT)

clean:
	@rm -f $(SIDE_EFFECTS)

$(AUX): $(TEX)
	@echo "Running pdflatex"
	@$(PDFLATEX) $(@:.aux=.tex)

$(BBL): $(TEX) $(BIB)
	@echo "Running bibtex"
	@$(BIBTEX) $(@:.bbl=.aux)

$(OUTPUT): $(TEX) $(BBL) $(PLOTS) $(FIGS)
	@echo "Running pdflatex"
	@$(PDFLATEX) $(@:.pdf=.tex) > /dev/null
	@$(PDFLATEX) $(@:.pdf=.tex) > /dev/null

#paper.pdf: paper.tex intro.tex problem.tex prioritized.tex results.tex related.tex conclusion.tex guava-small.eps guava-medium.eps guava-large.eps
#	pdflatex paper.tex

guava-small.eps guava-medium.eps guava-large.eps: graphs.plot
	gnuplot graphs.plot


==> old.tex <==

% Why dump the entire cache when memory is full? Why not just reclaim some of
% the cache entries in order to get back to some target size? Better yet, why
% not reclaim those entries according to the eviction policy of the cache
% itself.

This paper introduces \emph{Prioritized Garbage Collection}, a collection
algorithm and system that implements this solution. The key idea is that the
application can ask the garbage collector to bound the total amount of
space occupied by a data structure. This bound is expressed either in bytes
or as a percentage of the total heap. An essential feature of our system is
that the application can also dictate the order in which 

\noindent
Automatic memory management (garbage collection) eliminates a number of
insidious memory-related errors by relieving the programmer of the duty of
figuring out which objects to free and when. Most collectors are built on a very
simple policy: do a collection when resources are running low, and free only
those objects that are provably no longer in use. This policy leads to a
space-time tradeoff: collection becomes increasingly expensive as the size of
the program's data approaches the limit of available memory. A longstanding
issue in garbage collection, however, is how to support programming techniques,
such as caching and memoization, that have their own, often conflicting
space-time tradeoffs. 

Consider a software cache, one of the most common examples of such a
structure. The bigger the cache the higher the hit rate, but the larger the
memory footprint. In order to bound space usage most caches implementation a
eviction policy to keep only the most valuable entries that fit in the allotted
space.

Such space-sensitive policies are almost impossible to implement in a garbage
collected language. First, there are no effective mechanisms to determine the
memory footprint of a particular data structure. Ad hoc solutions, such as
requiring a ``getSize'' method on all objects are brittle and invasive; more
uniform solutions based on reflection or debugging interfaces are extremely
slow. As a result the cache has no way of knowing when resources are running low
and it needs to trigger the eviction policy. Second, while the cache can decide
which entries to evict (e.g., based on LRU ordering), it cannot actively reclaim
their space. Its only option is to null out their references and wait for the
garbage collector to run, which can actually make the problem worse if there are
subsequent hits to those entries. One solution is to build the cache using soft
references, which are cleared automatically by the collector when memory runs
low. This solution fails, however, because the collector is completely unaware
of the eviction policy. In fact, we found that many runtime systems simply clear
\emph{all} soft references when memory is exhausted, in effect clearing the
entire cache. What is needed is closer cooperation and communication between the
application and garbage collector.

In this paper we present \emph{Prioritized Garbage Collection}, a mechanism for
supporting the implementation of space-sensitive data structures and
policies. The key idea is that we provide an interface to tell the garbage
collector the relative value of keeping or trashing substructures (e.g., cache
entries), regardless of whether or not they are reachable in the heap. Given a
target space bound the collector reclaims these substructures \emph{in the order
  dictated by the policy}.


\noindent
Paper positioning:

\begin{itemize}

  \item A longstanding issue in automatic memory management is how to support
    programming techniques, such as caching and memoization, that have an
    inherent space-time tradeoff.

  \item These techniques manage the tradeoff using an eviction policy, which
    takes into account a number of factors when deciding whether or not to keep
    a data item. These factors might include the value of the data to the
    application (e.g. hit rate), the cost of recomputing it (or requesting it),
    and the amount of space it occupies relative to the available resources.

  \item The problem is that current managed runtime systems provide no effective
    mechanisms to implement these policies. 

  \item Programs cannot easily determine the memory cost of a data structure (to
    evaluate the policy), nor can they actively evict structures from memory (to
    enforce the policy).

  \item Existing mechanisms -- the special reference types -- are extremely
    blunt instruments, and widely shunned in the professional development
    community.

  \item In this paper we present \emph{Prioritized Garbage Collection}, in which
    the collector works cooperatively with the application to support
    application-specific memory management policies. 

  \item Two key mechanisms: GC size query and GC priority queue. 

  \item Using these mechanisms we built a space-aware cache we call a
    \emph{Stash}. Compared to widely-used alternatives, such as soft reference
    caches and fixed-length queues, the Stash performs orders of magnitude
    better. The more constrained memory is, the bigger the performance gap.

\item Online discussions indicate that programmers want this capability. Guava
  has a ``size'' or ``weight'' parameter, but the value must be determined by
  the specific cache implementation.

\end{itemize}

\noindent
Notes from discussion with Emery...

\begin{itemize}

  \item Scenarios: software cache, memoization, lazy evaluation, backtracking
    search.

  \item We need a story about why we use mark/sweep collection instead of
    generational (or some other more ``modern'' algorithm). (1) Mark/sweep is
    still prevalent in memory-constrained devices, (2) performance win is so
    big, the choice of GC algorithm doesn't matter.

  \item Experiments. Use heavy-tail distribution. Look at how memcached is
    evaluated. Maybe take a trace and adapt it to work with our system.

  \item We can view the size bound as a natural alternative to heap growth:
    instead of growing the heap based on memory/GC pressure, we'll evict the
    lowest priority memory items.

  \item Best possible straw-man: careful estimation of cache entry sizes to
    select LRU queue length. Still possible to underprovision (and get an
    out-of-memory error). Or overprovision and not be able to store as many
    entries (should result in lower hit rate). It depends a lot on the
    variability of entry sizes. Very hard to estimate -- even strings can share
    structure (either by interning, copy-on-write, or shared substrings).

\end{itemize}



==> priority.tex <==
\section{Priority-based Collection}

\noindent




\begin{itemize}

\item Idea: use the GC size query mechanism to compute the size of each cache
  entry and make that information available to the cache management and eviction
  policies.

\item The Guava cache includes a size-sensitive policy, but expects each entry
  type to implement its own sizing mechanism. The GC size query mechanism is
  perfectly complimentary because it can compute the size of any structure.

\item More sophisticated size-sensitive policies include the greedy-dual
  algorithm.

\item Basic algorithm: Create GC size query references for each cache
  entry. When the collector runs the sizes will be computed and the cache can
  evict entries that exceed the total size bound according to the eviction
  policy (LRU in our case).

\item Issue: what should be the order of size queries? Key idea: we want the
  size of the entry to represent accurately how much memory we would reclaim if
  it were evicted. That is only true if the size measurement represents the
  footprint reachable \emph{only} from the given object -- not from the roots,
  and not from any earlier queries. In other words if two entries share some
  internal structure, then the size query should charge that shared structure
  against the entry less likely to be evicted. It's fine if both are evicted,
  but if the entry charged with the shared region is the one evicted, the amount
  of memory reclaimed will not be accurate, since the region will be kept alive
  by the other entry.

\item Entries must be sized in order of possible eviction, from least likely to
  most likely. To support this requirement the system provides a size query
  queue, which the application can manage. At GC time the collector visits a set
  of size queries in the order specified in the queue. There may be multiple
  queues, but each query can reside in only one queue.

\item There is still a problem: eviction does not actually free any memory until
  the \emph{next} collection cycle. One collection is required to size the
  entries, which the Stash can use to perform evictions, but from user code
  performing an eviction simply means removing the objects. A second collection
  is required to reclaim the objects.

\item Ironically, eviction can actually make things worse! If there are requests
  for recently evicted entries the program can end up with two copies of the
  entry in memory (one evicted and unreachable and the other recreated to serve
  the cache request).

\item To address this problem we allow the garbage collector to perform the
  evictions. The Stash sets a total space bound on the query queue. The
  collector performs the size query closures in order, but stops when the bound
  is reached. Any remaining entries end up unmarked, and can therefore be
  reclaimed by the sweeper immediately.

\item The issue with this strategy is that entries could become partially
  reclaimed if there are external references into the middle of the
  structure. This is an issue with the size query mechanism as well, since
  external references can cut off the size computation. This mechanism is never
  unsafe, however, because it reclaims only those objects that are reachable
  from the cache entry and nowhere else.

\end{itemize}


We have a mechanism to get the size of objects in terms of bytes at
runtime. Specifically, given a collection of objects, we can figure out how much
memory the collection uses. With this, we can look at the Stashe, a structure
that can manipulate the collector to work with the logic of the programmer in
mind, rather than just liveness.

\subsection{Changes to GC}

Just as before, the virtual machine has a double-ended queue for the
queries. Along with the method to allow programmers to query the size of an
object (\lstinline{querySizeOf}), there are methods to manipulate the deque,
\lstinline{push} and \lstinline{remove}. We have added a \lstinline{long maxSize}, 
the maximum number of bytes of values the user-level Stashe can
keep.

The marking phase is unchanged. The closure phase now has a global
accumulator. If this accumulator exceeds \lstinline{maxSize} in the middle of
measuring an object, we abandon the closure and report a size of 0 bytes. The VM
removes all references from the query object to prevent dangling
pointers. Furthermore, we remove the value of local accumulator from the global
accumulator and move on to the next query. The collector will sweep the
remainder of this object. In this way, we free some memory that previously would
have stayed alive, but gone unused. The next collection will ultimately remove
the abandoned query.

\subsection{Data Structure}

Figure ~\ref{fig:stashe} details the Stashe class. The structure consists of
four parts, a map to store the key-value pairs, a map that relates keys to size
queries, a stack to keep track of the most recently used keys, and the maximum
number of bytes of values that can be stored.

\begin{figure}[t]
\begin{lstlisting}
class Stashe <K,V> {
  protected HashMap<K, V> map;
  protected HashMap<K, GCSize> sizeMap;
  protected Stack<K> stack;
  protected long currentSize, maxSize;

  public Stashe(long maxSize);

  public boolean put(K key, V value);
  public V get(K key);
  public V remove(K key);

  private void update();
}
\end{lstlisting}
\caption{Interface for \lstinline{Stashe} data structure}\label{fig:stashe}
\end{figure}

As with a cache built around a HashMap, we can \lstinline{put} key-value pairs
in, \lstinline{get} a value using a key, and \lstinline{remove} a value using a
key. The Stashe manipulates the dequeue in accordance with the least recently
used policy built in. When these three methods are called, we \lstinline{update}
to keep the structure inline with the last collection.

\paragraph{put} 
Given a key-value pair, the Stashe removes any previous key in the maps and the
stack. If the key is new, we query this value object and push it to the front of
the deque. If the value previously in the map is the same as the one to be
entered, the \lstinline{GCSize} object is reused and pushed to the front of the
deque. Otherwise, we remove the previous query from the collector's deque and
query the new object. This new query is pushed onto the front of the deque. In
all cases, the key is moved to the top of the stack, denoting it as the most
recently used key.

\paragraph{get} 
If there is a pair for a given key, we push the \lstinline{GCSize} query to the
front of the deque and the key to the top of the stack.

\paragraph{remove} 
If there is a pair for the key, the key-value pair is removed from the map, the
\lstinline{GCSize} object is removed from both the Stashe's map and the
collector's deque. Finally, the key is removed from the stack.

\paragraph{update} 
If any of the GCSize objects were updated, then a collection occured. We go
through the key-value map in order of the most recently used keys. If the
\lstinline{GCSize} query reports had size 0 after collection, we remove it from
the map. Otherwise, we keep it in the map. Note we do not have to check if we
exceed the \lstinline{maxSize} at this stage since the collector ensured we only
have \lstinline{maxSize} bytes of values after the garbage collection.



==> related2.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Reference Types}
Hayes introduced Ephemerons to determine unreachable objects in key-property lists instead of
using a list with a weak key and strong value~\cite{hayes97}. This capability allows entries
with dead keys to be removed from the list and properly deleted. We expect items in a
cache to be reachable only from the cache. Therefore, removing stale objects is not a
priority. Instead, we remove elements that cause our structure to exceed its limit.

%Work on Ephemerons ~\cite{hayes97}
%\begin{itemize}
%\item Finding key-value pairs that are unreachable and notifying them about death
%\item Useful for determining items in tables that can no longer be accessed
%\item Depends on the fact the key of those pairs is live in the program
%\item Keys for caches may not even exist until an outside source gives it to us
%\end{itemize}


%Related work in operating systems? Emery's GC without paging?

%Recent work on Haskell Resource Containers. ~\cite{yang14}
%\begin{itemize}
%\item Blocks of code regulated to containers that check memory usage.
%\item If limit exceeded, accompanying thread is killed.
%\item Security minded in sense that exceeding a limit is not expected behavior.
%\item We allow the limit to be exceeded, but when GC is run, reign it in.
%\item We want to maintain correctness and completion.
%\end{itemize}


%Resource Accounting for Java 1.2. ~\cite{czajkowski98}
%\begin{itemize}
%\item Interface for programmers to monitor resources threads use.
%\item Allow programmer to implement their own reaction to a thread exceeding resources.
%\item Insert bytecode in objects to obtain their size.
%\item Does not utilize the GC or memory allocator, which they admit would have cut down on% their overhead.
%\end{itemize}

\subsection{Programs Acting on Resource Limits}
There is a considerable body of work on caching for web traffic. The Greedy-Dual
algorithm takes into account the amount of time to obtain a page as well as the
size of the page to determine its eviction~\cite{cao97}. The cached objects are
text documents, so their size can be easily measured. Our system allows these
kinds of eviction policies to be used in general software caches, where measuring 
the size of a cached structure is non-trivial.

Yang and Mazi\`{e}res describe resource containers for Haskell that bound the
memory usage of untrusted code ~\cite{yang14}. Exceeding the limit of the
container kills the accompanying thread. A Sache is a more general structure,
which allows the program to choose what action to take when memory bounds are
exceeded. It could certainly be used to implement a security policy.

Czajkowski and von Eicken introduced an interface for programmers to monitor the
resources used by threads in a Java program~\cite{czajkowski98}. Furthermore,
they allow programmers to implement their own reaction to threads exceeding
their resource limits. They use bytecode rewriting to track heap memory usage
for each thread. In contrast, we track a list of known objects and use the
garbage collector to both track memory usage and enforce the limits. In
addition, our technique uses general heap reachability to define bounded
structures, rather than just thread ownership.

%Modeling workloads: prior studies have found that many aspects of Internet traffic follow Pareto distributions.
%\begin{itemize}
%\item Cunha, Bestavros, Crovella, ``Characteristics of WWW Client-based Traces''
%\item Atikoglu et al ``Workload Analysis of a Large-Scale Key-Value Store''
%\item Newman, ``Power laws, Pareto distributions and Zipf’s law''
%\end{itemize}

%Memory leaks in Java: many problems caused by caching (but what should we cite?)
%\begin{itemize}
%\item Mike Bond's work
%\end{itemize}

%Garbage Collector Memory Accounting in Language-Based Systems ~\cite{price03}
%\begin{itemize}
%\item Classify tasks in program
%\item Figure out how much memory attributed to a task by tracing heap
%\item We apply this idea to modify GC behavior and focus on a single task
%\end{itemize}

JAMM uses JVMTI to traverse the heap and compute the size of data
structures~\cite{jamm}.  This approach is flexible and powerful, but very
slow. A large data structure can require seconds of runtime to size (according
to the documentation). By piggybacking on the garbage collector we can perform
the same measurement with almost no performance overhead. The tradeoff, however,
is that we cannot compute sizes at arbitrary points during execution.

Price, Rudys, and Wallach divide a process into tasks and used the garbage
collector to track how much memory is attributed to each
task~\cite{price03}. Our work expands on this by allowing arbitrary data
structures to be tracked and by providing a way to enforce a size limit.

\cut{
GC Assertions allow programmers to efficiently check predicates about the
structure of the heap by using the garbage collector~\cite{aft09}. Our work
expands on this idea by allowing the program to interact with the garbage
collector in richer ways: asking quantitative questions, such as size, and
asking the collector to enforce policies.
}

\subsection{Using GC to Assist Running Programs}

O'Neill and Burton presented simplifiers as a way to improve the performance
of a program ~\cite{o'neill06simp}. Objects can add a \lstinline{simplify()} 
method that the garbage collector invokes when the collector traces over it.
With the measurement algorithm built into the collector, we can measure 
objects from existing libraries with no further modifications to those libraries.

The Data Structure Aware Garbage Collector lets the program denote which objects
are internal nodes for data structures~\cite{cohen15dsagc}. It uses this information 
to improve garbage collection for these structures and therefore overall performance.
Our work allows programs to run at points where the system would normally be out of
memory by changing the order of traversal.

%Other stuff:

%\begin{itemize}
%\item Two prior approaches to computing data structure size, one using JVMTI and
%  one using reflection. Performance is very poor, making them unsuitable for
%  production use.

%\item Soft references are not a good solution (and are discouraged in many
%  development communities) because the virtual machine has no knowledge about
%  the relative importance of keeping (or trashing) particular
%  structures. Existing systems typically implement a very simple policy: when
%  memory is exhausted all soft references are cleared. Our measurements show
%  that this policy performs very poorly and is only useful as an emergency
%  measure.
%\end{itemize}


==> size.tex <==
\section{GC Size Queries}

\noindent
One of the key challenges in implementing memory-sensitive algorithms is that it
is difficult (if not impossible) to compute the memory footprint of a data
structure. One problem is that there is no easy way to visit all the objects
that make up a structure (mostly due to encapsulation). Another problem is
making sure that shared structures are properly accounted. For example, if an
ArrayList contains 100 references to the same 32-byte object, we do not want to
report the structure size as 3200 bytes (plus the size of the array itself).

Our observation is that the garbage collector is ideally suited to compute this
information. The collector can follow all references regardless of
encapsulation, and visits each object exactly one time. We can piggyback the
size computation on the closure phase of the collection, adding only a tiny
amount of extra work. There are several issues and nuances with this strategy,
which we discuss below.

\subsection{Timing of size computations}

\noindent
The most obvious consequence of using the garbage collector to compute sizes is
that this information is only available after a collection, and it is only valid
as long as the structure is unchanged. We consider this limitation a reasonable
tradeoff given the extremely low overhead of the technique, particularly in
comparison to the alternatives (see Section~\ref{sec:results}). In addition, the
garbage collector tends to run more frequently right at the time that
memory-sensitive algorithms need more accurate information: when the system is
under memory pressure.

Since GC timing is asynchronous to the application, our interface treats size
computations like futures: the application issues a size query to the system,
which returns a future that \emph{will} contain the size information when
collector runs. A size query consists of a single object, which is the root of
the data structure to be sized. The garbage collector creates a new size future,
which it stores internally in addition to returning it to the application. When
the collector runs it computes the size of the structure, stores the result in
the future, and sets a flag on the future indicating that the information is
fresh. The application can either poll the future or block until the information
is ready. The interface does not currently support a callback, since that code
would be run in the GC thread. Below is an example of the interface in use:

\begin{small}
\begin{lstlisting}
// -- Issue a size query on the structure 
//    headed by o (the root)
GCSize q = System.sizeQuery(o);

// -- Check if the collector has run...
if (q.fresh()) {
    // -- If so, get the size information 
    //    (also resets the freshness flag)
    int size = q.get();

    // -- Do something with size
    if (size > threshold) {
        ...
    }
}
\end{lstlisting}
\end{small}

\subsection{Query semantics}

\noindent
A straightforward way to define the semantics of a size query is that it returns
the total number of bytes occupied by all objects reachable from the given query
root. This simple definition has a number of problems, however. 

First, we have found that typical Java heaps are much more connected than one
might expect. For example, many data structures have ``back references'' that
point from nodes back to their containers, effectively making all nodes
reachable from all other nodes. A size query on any node would always return the
size of the entire structure, which seems undesirable.

Second, there is a question about how to account for structure-sharing between
multiple size queries. Such sharing can occur in explicit ways (for example, by
having multiple indices into the same data) or in hidden ways (for example, if a
system interns strings). One answer is to consider each query independently and
count overlapping regions towards each relevant query. Implementing this
approach is problematic, though, because it might require the collector to visit
regions of the heap multiple times, changing the cost of collection. More
importantly, it would to combine size information because adding up the sizes
from multiple queries would not necessarily yield the total memory footprint.


% Say this? No attempt is made to invalidate size information if the heap is mutated

%\begin{itemize}
%
%\item The final issue is the timing. We do not trigger additional collections,
%  so size information is only as fresh as the last GC. For the purposes of
%  bounding resources this approach is reasonable, since resources cannot grow
%  indefinitely without triggering a GC.
%
%\item Since GCs are asynchronous from the standpoint of the application a GC
%  size query is treated like a future. The application creates a special
%  reference type for the queried object. The collector puts these reference
%  objects in a queue and processes them during a collection. The application can
%  check the reference object to see if the size information has been
%  computed. Once it retrieves the information an internal flag is reset until
%  the next GC.
%
%\end{itemize}



\subsection{Implementation}

\noindent
A straightforward way to compute structure sizes during collection is to
accumulate the sizes of objects visited during the closure phase. This strategy
can be implemented in a few different ways-- for example, by storing accumulated
size information in the work queue, and adding sizes as objects transition from
gray to black in the classic tricolor marking scheme.

The problem with this strategy is that it can yield wildly different results for
a given structure depending on the order of the heap traversal. The 


%\begin{itemize}
%
%\item This approach raises a second issue: what if there are multiple queried
%  objects and they share structure between them? We do not want to alter the
%  cost of GC, so we cannot visit the shared region twice. Counting it twice
%  would also interfere with our ultimate goal, which is to assess the overall
%  footprint of a set of objects, since adding up their sizes would not yield the
%  size of the whole structure.
%
%\item A consequence of our algorithm is that order matters: if two queried
%  objects share a region, the query that runs first will include the size of
%  this region; the one that runs second will not. In other words, any given
%  object in the heap is only counted towards a single query (whichever one
%  reaches it first). This approach maintains the important invariant that the
%  sum of all queried object sizes equals the footprint of all of the union of
%  all the objects involved.
%
%\end{itemize}

%\subsection{Reachable size vs dominating size}


\begin{itemize}

\item Idea: give the GC an object (the ``queried object'', ask it to compute the
  total size of all objects reachable from the object. We call this the
  ``reachable size''.

\item Basic implementation is straightforward: accumulate the sizes during the
  closure (marking) phase. There are a few ways to implement it (e.g., keep gray
  objects in the work queue). Adds very little overhead to the GC.

\item Big issue: structure sharing. The heap is not a tree.

\item One aspect: Java heaps are often more connected than you might
  think. ``All objects reachable'' is often much more than you want. Recall that
  the ultimate goal is to bound resources, so what we really want to know is how
  much memory we would get back if the object was reclaimed.

\item Instead we measure the footprint of objects reachable \emph{only} from the
  queried object. We call this metric the ``dominating size''.

\item To implement it we alter the order of the closure phase of the GC.  We
  start marking at the GC roots, as usual, but when we encounter a queried
  object we do not traverse any of its outgoing pointers. When the root closure
  is complete, we go back to the queried object and complete the closure from
  there, accumulating the sizes of any newly marked objects.

\end{itemize}



We augmented the MarkSweep garbage collector in Jikes RVM 3.1.2 to measure the
size of all items only reachable from a given object at each garbage
collection. This allows us to measure the size of data structures. We reuse the
mechanics of the MarkSweep collector to minimize the impact on both the runtime
of the program and collection time. The programmer calls the method
\lstinline{querySizeOf} with the object. They receive a \lstinline{GCSize}
object. This object holds a reference to the query object and will be filled in
with the size after a garbage collection. These are kept in a double-ended
queue, or deque, inside the VM.

\begin{figure}[t]
\begin{lstlisting}
class GCSize {
  protected long size;
  protected boolean fresh;
  protected ObjectReference query;
  
  public long getSize();
  public boolean isFresh();
}
\end{lstlisting}
\caption{Interface for \lstinline{GCSize} object}
\end{figure}
The measurement procedure is separated into two phases, query marking and query closure.

\paragraph{Query Marking}
The marking of query objects occurs right after the VM marks the root objects
and happens in the same way as the roots. The VM goes through each
\lstinline{GCSize} object in the queue and marks the query object each points to
as live. At the root's closure phase, if an object is marked as live, then the
VM does nothing to it. Therefore, when the VM encounters the query objects, it
will not attempt to mark any object past it. This leaves objects only reachable
from the queries unmarked.

\paragraph{Query Closure}
This closure occurs right after the closure for the roots. We perform the
closure for each reference in the queue. At each step, we accumulate the size of
the object currently observed. Once there are no other objects to look at, we
return the accumulator.

\begin{algorithm}
\caption{Query Closure Phase}\label{alg:qclosure}
\begin{algorithmic}
\Procedure{Query Closure}{$deque$}
\ForAll{$gcsize\in deque$}
	\State $values=\emptyset$
	\State $values.push(gcsize.query)$
	\Repeat
		\State $o\gets values.pop()$
		\State $gcsize.size\gets gcsize.size + sizeOf(o)$
		\ForAll{objects $p$ that $o$ points to}
			\If{ $p$ is not live }
				\State mark $p$ as live
				\State $values.push(p)$
			\EndIf
		\EndFor
	\Until{$values ==\emptyset$ }
	\State $gcsize.fresh = true$
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Properties}
If we measure a single structure, the size we retrieve tells us how many bytes
are taken up by the structure. Let us think of a structure $S$ as a set of
objects, where each object may itself be a structure. Then the size of $S$ is at
most the sum of the size of all the objects in $S$.

$$size(S) = \sum_{i = 0}^{|S|}{size(o_i)}$$

When we measure more than one object per GC, the order they are queried in can
affect the size measured. Let us query objects $o1$ and $o2$ in that order. Let
$o1$ and $o2$ both point to a third object $p$. The query closure, like the root
closure, ignores marked objects. Therefore, $o_2$ will not consider any objects
reachable from $p$. Then,

$$size(o_1) = size(o_1\backslash p) + size(p)$$
$$size(o_2) = size(o_2\backslash p)$$

This leads to the size $o_2$ not reflecting how much memoryit is actually
using. However, the sum reflects how much memory is in use by all of the query
objects.

$$size(o_1) + size(o_2) = size(o_1\backslash p) + size(p) + size(o_2\backslash p)$$

This is the crux of the Stashe, an assurance that we can state how much memory a
collection of structures is using.


==> stuff.tex <==
% \begin{itemize}

% \item Problems: (1) hard to size a cache effectively by number of
%   entries, and (2) conflicting time/space tradeoffs for caches and GC.

% \item Soft references: solution of last resort -- blows everything away,
%   with no accounting of the value of data.

% \item Solution: Bounded-size cache. Solves (1) by making the best use of
%   the available space. More entries if they fit; fewer if they
%   don't. Addresses (2) because it the bound can be used to avoid creating
%   memory pressure.

% \item Key idea: pass information to the GC so that it can enforce the bound
%   in a way that respects the relative value of the data.

% \end{itemize}

\textbf{NOTES:}

Big things to do:

\begin{itemize}

\item Different title? Maybe ``Garbage Collector Support for Software Caches''

\item Add memcached experiments

\item Maybe add the memory leak experiment?

\item Figure out how to describe the GC interface

\item Figure out how to evaluate the adaptive algorithm -- do we need another
  workload going on in the program in order to show the adaptivity?

\end{itemize}

The GCSizeQuery supports implementation of any cache algorithm that needs to
know the size of a cache entry. The other problem for caches implemented in Java
is capacity. What should the capacity be?

\begin{itemize}

\item Overall, larger is better for cache hits

\item GC costs grow relatively slowly until there is memory pressure

\item We could have a target amount of free space? Maximizes size.

\item Is there cost function we could use to do gradient descent? Overall
  performance seems like the obvious choice, but it's mixed up in all the other
  things going on in the program.

\item One low end: start small, grow the cache and measure improvement in hit rate.

\item Problem: we always let the cache grow, then evict back down to the target
  size.

\item Is there some notion of a total value for the cache? Add up cost(p) for
  each entry p?

\item Top end: Cannot let memory pressure occur. Makes sense with a target for
  free memory. Maybe driven by the heap growth function.

\item Could we use memory pressure as a penalty factor in the cost model?

\end{itemize}

Potential algorithm:

\begin{itemize}

\item Given a sash with size X\% of the heap.

\item Mark all objects reachable from roots, skipping the objects in the
  sash. Computes a precise live size of the non-sash heap. Call it Y\%

\item Let C\% be a safe amount of reserve in the heap

\item If X+Y+C < 100 then no change

\item If X+Y+C << 100 then increase X. We can measure the change in hit rate to
  see if it is helping.

\item If X+Y+C > 100 then reduce X by the amount over (X+Y+C-100). We can
  measure the GC frequency and reduce it by more.

\item It probably doesn't make a lot of sense to shrink the sache size
  significantly, since any cache algorithm can be set to use a small number of
  entries. The interesting question is on the upper end of the size.

\end{itemize}


\TBD{For the intro: many web caching algorithms developed over the years take
  into account the size of the items begin cached (e.g., greedy-dual-size and
  related algorithms). Getting the size can be hard (in any language) when the
  items being cached are not simple values like strings.}

\TBD{The hard problem is figuring out how *big* the cache can be without causing
  GC thrashing or paging}

\TBD{More broadly, being able to bound the total memory footprint of a data
  structure is useful for many things -- memory leaks, hacker attacks}

% ----------------------------------------------------------------------

\begin{itemize}

\item Software caching is hard to implement well in a garbage collected
  language.

\item Core problem in caching: get the highest hit rate for a given storage
  budget. And in general, the bigger the budget the better the hit rate.

\item Key issue: how to size the cache? We want to make the cache big, but but
  not so big that it creates memory pressure and soaring GC costs. We don't want
  to trigger emergency GC behavior (e.g., clear all soft references, or expand
  the heap and start paging).

\item Existing caches measured in number of entries. But what if values being
  cached are wildly different sizes? Could be determined in an ad-hoc way, but
  hard to implement with encapsulation; easy to get wrong.

\item Problems:

\item (1) No general way to measure and bound the memory use of a data structure.

\item (2) No way to detect and respond to memory pressure.

\item Problem: interaction between cache and GC. Under pressure we could expand
  the heap or shrink the


\item For such workloads many eviction policies take into account the size of
  the individual values being cached.

\item Even worse: eviction doesn't work.

\end{itemize}



% ----------------------------------------------------------------------

